Learning to Find Usages of Library Functions in Optimized Binaries

Much software, whether beneficent or malevolent, is distributed only as binaries, sans source code. Absent source code, understanding binaries' behavior can be quite challenging, especially when compiled under higher levels of compiler optimization. These optimizations can transform comprehensible, "natural" source constructions into something entirely unrecognizable. Reverse engineering binaries, especially those suspected of being malevolent or guilty of intellectual property theft, are important and time-consuming tasks. There is a great deal of interest in tools to "decompile" binaries back into more natural source code to aid reverse engineering. Decompilation involves several desirable steps, including recreating source-language constructions, variable names, and perhaps even comments. One central step in creating binaries is optimizing function calls, using steps such as inlining. Recovering these (possibly inlined) function calls from optimized binaries is an essential task that most state-of-the-art decompiler tools try to do but do not perform very well. In this paper, we evaluate a supervised learning approach to the problem of recovering optimized function calls. We leverage open-source software and develop an automated labeling scheme to generate a reasonably large dataset of binaries labeled with actual function usages. We augment this large but limited labeled dataset with a pre-training step, which learns the decompiled code statistics from a much larger unlabeled dataset. Thus augmented, our learned labeling model can be combined with an existing decompilation tool, Ghidra, to achieve substantially improved performance in function call recovery, especially at higher levels of optimization.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> tables/comparison.tex <==
\toufique{Evaluation criteria: We tracked down all the functions having at least one marker. We generated the blocks following the same rule as before (20 lines block with shift 3) and associated each block to the corresponding markers. That means if a block has multiple markers, we associate that block with each marker. Therefore, at the end of the process, we have a list of candidate blocks for each marker. We applied our model to the blocks. Correct: the model predicts the target function for at least one block and predicts no label for other blocks. Partial: the model predicts the target function for at least one block and wrong function for one block. We will get high partials where the density of markers is high. Incorrect: the model fails to predict the target function for all blocks. I will recheck the last two columns. I have some idea to check that in a different way.}


\begin{table}[h]

\centering
\resizebox{\columnwidth}{!}{%
\renewcommand{\arraystretch}{1.2}% Tighter


\begin{tabular}{|C{1cm}|C{1cm}|C{1cm}|C{1cm}|C{1cm}|C{1cm}|C{1cm}|C{1cm}|C{1cm}|}
\hline
\multirow{2}{1cm}{\textbf{OPT-level}} & \multirow{2}{1cm}{\textbf{Number of file processed}} & \multirow{2}{1cm}{\textbf{Markers in ghidra (inline functions)}} & \multicolumn{4}{c|}{\textbf{Satyanweshi}}                                                                 & \multirow{2}{1cm}{\textbf{Function Recovered by Hexray}} & \multirow{2}{1cm}{\textbf{Unique Function Recovered by Hexray}} \\ \cline{4-7}
                                             &                                                    &                                                                & \textbf{Correct} & \textbf{Partial Correct} & \textbf{Failure/ Wrong} & \textbf{Unique Function Recovered} &                                                         &                                                                \\ \hline
O1                                           & 30                                                 & 319                                                            & 242              & 25                       & 52                     & 7                                  & 4                                                       & 2                                                              \\ \hline
O2                                           & 196                                                & 1731                                                           & 874              & 345                      & 512                    & 68                                 & 84                                                      & 20                                                             \\ \hline
Os                                           & 197                                                & 2082                                                           & 1514             & 196                      & 372                    & 47                                 & 75                                                      & 19                                                             \\ \hline
O3                                           & 144                                                & 2301                                                           & 1175             & 400                      & 726                    & 55                                 & 72                                                      & 14                                                             \\ \hline
Of                                           & 150                                                & 2388                                                           & 1349             & 466                      & 573                    & 34                                 & 57                                                      & 17                                                             \\ \hline

\end{tabular}

}
\end{table}

==> tables/optimization_tables.tex <==
\renewcommand{\arraystretch}{1.5}

\begin{table}[h!]
    \begin{tabular}{l|p{6cm}}
    \hline
    \textbf{Optimization level} & \textbf{Description}                                                                                                                                                   \\
    \hline
    -O0                & Default optimization, fastest compile time                                                                                                       \\
    -O1 (or -O)        & Optimizes for code size and execution time; somewhat longer compile time                                                                              \\
    -O2                & Performs more optimizations that O1 such as inlining functions with the aim of increasing performance while greatly increasing compile time                     \\
    -O3                & Introduces more optmizations than O2 such as loop unrolling, trading code size, memory usage and compile time for better runtime performance                    \\
    -Os                & Enables the same optimizations as O2 except those that increase code size (such as function alignment), but does inline functions when optimizing for code size \\
    -Ofast             & Disregards strict standard compliance while enabling all O3 optimizations\\
    \hline                                                                                      
    \end{tabular}
    \caption{Overview of optimization levels provided by the gcc and g++ compilers \label{tab:optimization}}
    \end{table}

==> tables/result_validation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]

\centering
\resizebox{\columnwidth}{!}{%
\renewcommand{\arraystretch}{1.6}% Tighter

\begin{tabular}{|L{1.5cm}|L{1.5cm}|L{1.5cm}|L{1.5cm}|l|c|c|c|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{1.5cm}{\textbf{Experimental Setup}}} 



& \multicolumn{1}{c|}{\multirow{2}{1.5cm}{\textbf{Model}}} 
& \multicolumn{2}{c|}{\multirow{2}{1.5cm}{\textbf{Averaging Criteria}}}
& \multicolumn{1}{c|}{\multirow{2}{1.5cm}{\textbf{Mean/ C.I. @95\%}}} 

& \multirow{2}{*}{\textbf{Prec.}} & \multirow{2}{*}{\textbf{Recall}} & \multirow{2}{*}{\textbf{F-score}} \\
\multicolumn{1}{|c|}{}                                             & \multicolumn{1}{c|}{}                                & \multicolumn{2}{c|}{}                                             & \multicolumn{1}{c|}{}                                           &                                     &                                  &                                     \\ \hline
\multirow{9}{1.5cm}{No Filtering}                                      & \multirow{3}{*}{Block}                               & \multicolumn{2}{l|}{micro}                                        & NA                                                              & 0.9421                               & 0.9421                            & 0.9421                               \\ \cline{3-8} 
                                                                   &                                                      & \multicolumn{2}{l|}{macro}                                        & NA                                                              & 0.3123                               & 0.3162                            & 0.2973                               \\ \cline{3-8} 
                                                                   &                                                      & \multicolumn{2}{l|}{weighted}                                     & NA                                                              & 0.9402                               & 0.9421                            & 0.9402                               \\ \cline{2-8} 
                                                                   & \multirow{6}{*}{Prior}                               & \multicolumn{2}{l|}{\multirow{2}{*}{micro}}                       & Mean                                                            & 0.7892                               & 0.7892                            & 0.7892                               \\ \cline{5-8} 
                                                                   &                                                      & \multicolumn{2}{l|}{}                                             & C.I. @95\%                                                      & .7890-.7893                         & .7890-.7893                      & .7890-.7893                         \\ \cline{3-8} 
                                                                   &                                                      & \multicolumn{2}{l|}{\multirow{2}{*}{macro}}                       & Mean                                                            & 0.0035                               & 0.0035                            & 0.0034                               \\ \cline{5-8} 
                                                                   &                                                      & \multicolumn{2}{l|}{}                                             & C.I. @95\%                                                      & .0034-.0035                         & .0034-.0035                      & .0034-.0034                         \\ \cline{3-8} 
                                                                   &                                                      & \multicolumn{2}{l|}{\multirow{2}{*}{weighted}}                    & Mean                                                            & 0.8354                               & 0.7892                            & 0.8116                               \\ \cline{5-8} 
                                                                   &                                                      & \multicolumn{2}{l|}{}                                             & C.I. @95\%                                                      & .8353-.8354                         & .7890-.7893                      & .8115-.8117                         \\ \hline
\multirow{9}{1.5cm}{Discarding true positive for no label class}       & \multirow{3}{*}{Block}                               & \multicolumn{2}{l|}{micro}                                        & NA                                                              & 0.4763                               & 0.4763                            & 0.4763                               \\ \cline{3-8} 
                                                                   &                                                      & \multicolumn{2}{l|}{macro}                                        & NA                                                              & 0.3053                               & 0.3092                            & 0.2903                               \\ \cline{3-8} 
                                                                   &                                                      & \multicolumn{2}{l|}{weighted}                                     & NA                                                              & 0.4685                               & 0.4763                           & 0.4637                               \\ \cline{2-8} 
                                                                   & \multirow{6}{*}{Prior}                               & \multicolumn{2}{l|}{\multirow{2}{*}{micro}}                       & Mean                                                            & 0.0034                               & 0.0034                            & 0.0034                               \\ \cline{5-8} 
                                                                   &                                                      & \multicolumn{2}{l|}{}                                             & C.I. @95\%                                                      & 0033-.0034                          & .0033-.0034                      & .0033-.0034                         \\ \cline{3-8} 
                                                                   &                                                      & \multicolumn{2}{l|}{\multirow{2}{*}{macro}}                       & Mean                                                            & .00029                              & .00044                           & .00032                              \\ \cline{5-8} 
                                                                   &                                                      & \multicolumn{2}{l|}{}                                             & C.I. @95\%                                                      & .00028-.00030                       & .00040-.00046                    & .00030-.00033                       \\ \cline{3-8} 
                                                                   &                                                      & \multicolumn{2}{l|}{\multirow{2}{*}{weighted}}                    & Mean                                                            & 0.0032                               & 0.0034                            & 0.0032                               \\ \cline{5-8} 
                                                                   &                                                      & \multicolumn{2}{l|}{}                                             & C.I. @95\%                                                      & .0031-.0033                         & .0033-.0034                      & .0031-.0032                         \\ \hline
\end{tabular}
}
\end{table}
